Existence of arbitrary large numbers of non-$\mathbb R$-covered Anosov flows on hyperbolic $3$-manifolds

The purpose of this paper is to prove that, for every $n\in \mathbb N$, there exists a closed hyperbolic $3$-manifold $M$ which carries at least $n$ non-$\mathbb R$-covered Anosov flows, that are pairwise orbitally inequivalent. Due to a recent result by Fenley, such Anosov flows are quasi-geodesic. Hence, we get the existence of hyperbolic $3$-manifolds carrying many pairwise orbitally inequivalent quasi-geodesic Anosov flows. One of the main ingredients of our proof is a description of the clusters of lozenges that appear in the orbit spaces of the Anosov flows that we construct. The number of lozenges involved in each cluster, as well as the orientation-type of this cluster, provide powerful dynamical invariants allowing to prove that the flows are orbitally inequivalent. We believe that these dynamical invariants could be helpful in a much wider context.

==> homeomorphic.tex <==
We will now prove item (4) of Theorem~\ref{t.con}. In view of Proposition~\ref{p.relation-alpha-beta}, it is equivalent to prove:

\begin{proposition}\label{p.h1}
For $m=1,\dots,2n$, there exists a homeomorphsim $h^m_\psi: W_\psi^m \longrightarrow W_\psi^0$ such that $h_\psi^m(W^s_{loc}(\widebar\apha_j^m))= W^s_{loc}(\widebar\apha_j^0)$ for every $j\in \{1,\dots, 2n\}$.
\end{proposition}

Let us briefly recall our notations. For $m=0,\dots,2n$, we have defined an explicit gluing diffeomorphism $\psi^m:\partial^{out} U\to\partial^{in}U$, considered the flow $Y_{\psi,t}^m$ induced by $X_t$ on the quotient manifold $W_\psi^m=U/\psi^m$. Although $Y_{\psi,t}^m$ is not necessarily an Anosov flow, it preserves two transverse foliations $\cF^{s,m}_{\psi}$ and $\cF^{s,m}_\psi$. We have constructed $2n$ some periodic orbits $\widebar\apha_1^m,\dots,\widebar\apha_{2n}^m$ of the flow. We denote by $W^s_{loc}(\widebar\apha_j^m)$ a tubular neighborhood of the periodic orbit $\widebar\apha_j^m$ in the leaf of $\cF_\psi^{s,m}$ containing this orbit. We recall that this is an abuse of notation, since $W^s_{loc}(\widebar\apha_j^m)$ is not necessarily a local stable set of $\widebar\apha_j^m$. 

The proof of Proposition~\ref{p.h1} is quite long, and will be divided into several steps. We fix an integer $m=1,\dots,2n$ for the remainder of the section.


\subsubsection{Preliminary: tunnels and ribbons in good positions in a tunnel.}  Let $D^s$ be a stable strip of $(U,X)$ \emph{i.e.} a connected  component of $\partial^{in}U\setminus\cL^s$. Since $D^s$ is disjoint form $W^s(\Lambda)$, the forward orbit of any point $x\in D^s$ will eventually exit $U$ at some point $\Theta(x)=X^{T(x)}(x)\in\partial^{out}U$. Note that $D^u=\Theta(D^s)$ is an unstable strip, \emph{i.e.} a connected component of $\partial^{out} U\setminus\cL^u$. Let 
$$E=\{X^t(x), x\in D^s, 0\leq t\leq T(x)\}$$
be the union of the orbit segments going from $D^s$ to $D^u$ in $U$. We call $E$ the \emph{tunnel} joining $D^s$ to $D^u$. One can easily verify that such a tunnel is homeomorphic to $\RR^2\times [0,1]$ through a homeomorphism mapping $D^s$ to $\RR^2\times\{0\}$, mapping $D^u$ to $\RR^2\times\{1\}$, mapping the orbits of the flow $X_t$ in $E$ to the vertical  segments $\{(\cdot,\cdot)\}\times [0,1]$, mapping the leaves of the stable foliation $\cF^s\cap E$ to the vertical bands $\{\cdot\}\times\RR\times [0,1]$ and mapping the leaves of the unstable foliation $\cF^s\cap E$ to the vertical bands $\RR\times\{\cdot\}\times [0,1]$.

Consider a \emph{ribbon} in $E$, \emph{i.e.} the image an embedding $R:[-1,1]\times [0,1]\hookrightarrow E\simeq \RR^2\times [0,1]$. We call $R([-1,1]\times\{0\})$ and $R([-1,1]\times\{1\})$ the \emph{ends} of the ribbon $R$. We say that this ribbon $R$ is \emph{in good position} (with respect to the foliation $\cF_\psi^{s,0}$) if there exists a function $r_s:[0,1]\to\RR$ such that 
$$\forall t\in[0,1], \quad R([-1,1]\times\{t\})\subset \{r_s(t)\}\times\RR\times\{t\}.$$
Observe that this definition implies that for every $t\in[0,1]$, the arc $R([-1,1]\times\{t\})$ must be included in a leaf of the foliation $\cF^s\cap E$. This also implies that one of the two ends of $R$ must be included in $D^s$ and the other must be included $D^u$ respectively. The following fact is a immediate consequence of he convexity of the set of ribbons which are in good position in $E$ for the natural affine structure on $E\simeq \RR^2\times [0,1]$:

\begin{fact}
\label{f.ribbons-isotopic}
Let $R,R'$ be two ribbons in good positions in a tunnel $E$, with the same ends. Then $R$ and $R'$ are isotopic, with fixed ends, among ribbons in good position.
\end{fact}

\subsubsection{Step 1. Construction of an explicit diffeomorphism $\bar h_\epsilon:W^m_\psi\to W_\psi^0$.} Recall that the gluing maps $\psi^0,\psi^m$ were defined by the formulae
$$\psi^0_{|T_i^{out}}=\tau_{+1/2}\circ\sigma\quad\mbox{and}\quad\psi^m_{|T_i^{out}}=\left\{\begin{array}{ll}\tau_{-1/2}\circ\sigma & \mbox{if }i\leq 2m\\\tau_{+1/2}\circ\sigma & \mbox{if }i>2m\end{array}\right.$$
where $\tau_{v}$ is the translation $(x,y)\mapsto (x+v,y)$ in the coordinate system $\xi_i:T_i^{in}\to \TT_i=(\RR/(2i+2)\ZZ)\times(\RR/\ZZ)$. As a consequence, 
$$\psi^m_{|T_i^{out}}=\left\{\begin{array}{ll}\tau_{-1}\circ\psi^0_{|T_i^{out}} & \mbox{if }i\leq 2m\\ \psi^0_{|T_i^{out}} & \mbox{if }i>2m\end{array}\right.$$
One may add a coordinate $t$ in order the coordinates $(x,y)$ in order to obtain a coordinate system $(x,y,t)\in (\RR/(2i+2)\ZZ)\times(\RR/\ZZ)\times [0,1]$ on a collar neighborhood $V_i$ of the torus $T_i^{in}$ in the $3$-manifold $U$. One can choose the coordinate $t$ so that the torus $T_i^{in}$ corresponds to $\{t=0\}$, and the vector field $X$ corresponds to $\frac{\partial}{\partial t}$. Given $\epsilon\in ]0,1]$, we denote by $V_{i,\epsilon}$ the part of $V_i$ corresponding to $t\in [0,\epsilon]$ in the $(x,y,t)$ coordinate system. Then we define a homeomorphism $h_\epsilon:U\to U$ by setting:
$$h_{\epsilon}(x,y,t)=\left(x+1-\frac{t}{\epsilon},y,t\right)\mbox{ on }V_{i,\epsilon}\mbox{ for }i=1,\dots,2m\mbox{ and }
h_\epsilon=\mathrm{Id}\mbox{ on }U\setminus \cup_{i=1}^{2m} V_{i,\epsilon}.$$
Notice that $h_{\epsilon}=\tau_{-1}^{-1}$ on $T_i^m$ for $i\leq 2m$, $h_{\epsilon}=\mathrm{Id}$ on $T_i^m$  for $i>2m$, and  $h_{\epsilon}=\mathrm{Id}$ on $T_i^{out}$ for every $i$. It follows that $h_{\epsilon}\circ \psi^m=\psi^0\circ h_\epsilon$. As a consequence, $h_\epsilon$ induces a diffeomorphism 
$$\bar h_\epsilon:W_\psi ^m=U/{\psi^m}\longrightarrow W_\psi^0=U/\varphi^0.$$  

\medskip

\noindent\textit{\textit{Some notations.}} Using the diffeomorphism $\bar h_\epsilon$ (for a given $\epsilon$), we can map the ribbons $W^s_{loc}(\widebar\apha_1^m),\dots, W^s_{loc}(\widebar\apha_{2n}^m)$ in $W_\psi^0$. Then we  are left to prove that the ribbon links $W^s_{loc}(\widebar\apha_1^0) \cup \dots \cup W^s_{loc}(\widebar\apha_{2n}^0)$ and $\bar h_\epsilon(W^s_{loc}(\widebar\apha_1^m))\cup \dots \cup \bar h_\epsilon(W^s_{loc}(\widebar\apha_{2n}^m))$ are isotopic in $W_\psi^0$. In practice, we will describe an isotopy between $\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$ and $W^s_{loc}(\widebar\apha_{j}^0)$ for every $j$, so that the supports of the isotopies corresponding to the different integers $j$ are pairwise disjoint. One may already observe that, the ribbons $\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$ and $W^s_{loc}(\widebar\apha_{j}^0)$ coincide for $j>2m$. This follows from two facts: first, we know that $(\pi_\psi^0)^{-1}(\widebar\apha^j_0)=(\pi_\psi^m)^{-1}(\widebar\apha_j^m)$ for $j>2m$ (see Remark \ref{r.beta-indep-m}), and second, we observe that $(\pi_\psi^0)^{-1}(\widebar\apha^j_0)=(\pi_\psi^m)^{-1}(\widebar\apha_j^m)$ is disjoint from the support of the  diffeomorphism $h_\epsilon$ for $j>2m$. As a consequence, we will focus our attention on the case $j\leq 2m$.
 
\medskip

Until the very last step of the proof, we fix an integer $j\in\{1,\dots,2m\}$. For sake of simplicity, we will denote 
$$A:=W^s_{loc}(\widebar\apha_{j}^0)\mbox{ and }B_\epsilon:=\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m)).$$  
The tori $T_{\psi,2j-1}^0=\pi_\psi^0(T_{2j-1}^{in})=\pi_\psi^0(T_{2j-1}^{out})$ and $T_{\psi,2j}^0=\pi_\psi^0(T_{2j}^{in})=\pi_\psi^0(T_{2j}^{out})$ we will play a central role in the remainder of the proof. Fro $i=2j-1,2j$, we consider the one-dimensional foliation $f^{s,0}_{\psi,i}=\psi_\psi^0(f^{s,in}_i)=\psi_\psi^0(f^{s,out}_i)$ and $f^{u,0}_{\psi,i}=\psi_\psi^0(f^{u,in}_i)=\psi_\psi^0(f^{u,out}_i)$) on the torus $T_{\psi,i}^0$. Recall that we have constructed some stable and unstable strips
$$D_{2j-1}^s\subset A_{2j-1}^{1,s},\quad D_{2j-1}^u\subset A_{2j-1}^{1,u},\quad 
D_{2j}^s\subset A_{2j}^{1,s},\quad D_{2j}^u\subset A_{2j}^{1,u}$$
so that 
$$D_{2j-1}^u=\sigma(D_{2j-1}^s),\quad D_{2j}^u=\sigma(D_{2j}^s),\quad D_{2j-1}^u=\Theta(D_{2j}^s),\quad  D_{2j}^u=\Theta(D_{2j-1}^s).$$ 
See Proposition~\ref{p.selection-strips}. We denote by $E_j^+$ the tunnel joining the stable strip $D^s_{2j}$ to the unstable strip $D^u_{2j-1}$ in $U^+$, and by $E_j^-$ the tunnel joining the stable strip $D^s_{2j-1}$ to the unstable strip $D^u_{2j}$ in $U^-$. 

Using the definition of the basis $(\vec{e_1},\vec{e_2}, \vec{e_3})$ in Proposition~\ref{p.orient} and the definition of the translation $\tau_{-1}$ in section~\ref{sss.construction-psi}, one can check that the orientations of the Reeb annuli, the cyclic order of these annuli, and the orientation of the translation $\tau_{-1}$ on the tori $T_{\psi,2j-1}^0$ and $T_{\psi,2j}^0$ are just as depicted on Figure~\ref{f.strips} below. 

\begin{figure}[ht]
\centerline{\includegraphics[width=12cm]{Strips.eps}}
\caption{\label{f.strips}The tori $T_{\psi,2j-1}^0$ and $T_{\psi,2j}^0$, the strips $\pi_\psi^0(D_{2j-1}^s)$, $\pi_\psi^0(D_{2j-1}^u)$, $\pi_\psi^0(D_{2j}^s)$ and $\pi_\psi^0(D_{2j}^u)$, the direction of the vector field $Y^0$ and the direction of the translation $\tau_{-1}$.}
\end{figure}

\subsubsection{Step 2. Decomposition of the ribbon $A=W^s_{loc}(\widebar\apha_{j}^0)$.} We decompose $A$ in two halves 
$$A=A^+\cup A^- \mbox{ where } A^-:=A\cap \pi_\psi^0(U^-)\mbox{ and }A^+:=A\cap \pi_\psi^0(U^+).$$
We will now describe more precisely $A^+$ and $A^-$. For that purpose, recall that, the periodic orbit $\widebar\apha_j^0$:
\begin{itemize}
\item[--] intersects the torus $T_{\psi,2j-1}^0$ at a single point $\bar q_{2j-1}^0\in \pi_\psi^0(D_{2j-1}^s)\cap \pi_\psi^0(D_{2j-1}^u)$,
\item[--] intersects the torus $T_{\psi,2j}^0$ at a single point $\bar q_{2j}^0\in \pi_\psi^0(D_{2j}^s)\cap \pi_\psi^0(D_{2j}^u)$,
\item[--] does not intersect the torus $T_{\psi,i}^0$ for $i\neq 2j-1,2j$. See Proposition~\ref{p.construction-beta}.
\end{itemize}
Let $\ell^s(\bar q_{2j-1}^0)$  be the leaf of the foliation $f^{s,0}_{2j-1}$ containing the point  $\bar q_{2j-1}^0$ and $\ell^s(\bar q_{2j}^0)$  be the leaf of the foliation $f^{s,0}_{2j}$ containing the point $\bar q_{2j}^0$. Let
 $$I^s(\bar q_{2j-1}^0)=A\cap T_{\psi,2j-1}^0 \quad\mbox{and}\quad I^s(\bar q_{2j}^0)=A\cap T_{\psi,2j}^0.$$ 
 Clearly, $I^s(\bar q_{2j-1}^0)$ is a neighborhood of $\bar q_{2j-1}^0$ in $\ell^s(\bar q_{2j-1}^0)$, and $I^s(\bar q_{2j}^0)$ is a neighborhood of $\bar q_{2j}^0$ in  $\ell^s(\bar q_{2j}^0)$. Adjusting the width of $A$ if necessary, we may assume that $I^s(\bar q_{2j-1}^0)$ is a crossbar\footnote{By such we mean that the arc $I^s(\bar q_{2j-1}^0)$ is included in the unstable strip $\pi_\psi^0(D^u_{2j-1})$ and that the ends of $I^s(\bar q_{2j-1}^0)$ belong to the two boundary leaves of $\pi_\psi^0(D^u_{2j-1})$.} of the unstable strip $\pi_\psi^0(D^u_{2j-1})$, and $I^s(\bar q_{2j}^0)$ is a crossbar of the unstable strip $\pi_\psi^0(D^u_{2j})$. By definition, $A^-$ is a ribbon joining $I^s(\bar q_{2j-1}^0)$ to $I^s(\bar q_{2j}^0)$ in $U^-$ and $A^+$ is a ribbon joining $I^s(\bar q_{2j}^0)$ to $I^s(\bar q_{2j-1}^0)$ in $U^+$.  See Figure~\ref{f.decomposition-A}. Since $\bar q_{2j-1}^0\in \pi_\psi^0(D_{2j-1}^s)$ and $\bar q_{2j}^0\in \pi_\psi^0(D_{2j}^s)$, $A^+$ is contained in the tunnel $E^+_j$ and $A^-$ is contained in the tunnel $E_j^-$.
 
 \begin{figure}[ht]
\centerline{\includegraphics[width=13cm]{Decomposition-A.eps}}
\caption{\label{f.decomposition-A}Decomposition of the closed ribbon $A=W^s_{loc}(\widebar\apha_j^0)$.}
\end{figure}

\begin{remark}
\label{r.faithful}
Close to the tori $T_{\psi,2j-1}^0$ and $T_{\psi,2j}^0$, we have at our disposal some local coordinate systems  in which the flow $Y^0_t$, the foliations $f^{s,0}_{i}=\cF_\psi^{s,0}\cap T_{\psi,i}^0$ and $f^{u,0}_{i}=\cF_\psi^{u,0}\cap T_{\psi,i}^0$ and the translation $\tau_{-1}$ have a fully explicit simple form. As a consequence, our figures above and below represent quite faithfully the geometry of the ribbons $A=W^s_{loc}(\widebar\apha_j^0)$ and $B_\epsilon=\bar h_\epsilon(W^s_{loc}(\widebar\apha_{2j}^m))$ close to the tori $T_{2j-1}^0$ and $T_{2j}$. On the contrary, we do not pretend to be able to represent faithfully the geometry and topology of the ribbons far from $T_{\psi,2j-1}^0$ and $T_{\psi,2j}$.
\end{remark}

\subsubsection{Step 3. Decomposition of the ribbon $B_\epsilon=\bar h_\epsilon(W^s_{loc}(\widebar\apha_{2j}^m))$.} We cut $B_\epsilon$ into four pieces:
$$B_\epsilon=B_{2j,\epsilon}\cup B_{+,_\epsilon}\cup B_{2j-1,\epsilon}\cup B_{-,\epsilon}$$ 
where
$$B_{2j,\epsilon}:=B_\epsilon\cap V_{2j,\epsilon},\quad B_{2j-1,\epsilon}:=B_\epsilon\cap V_{2j-1,\epsilon}$$
$$B_{+,\epsilon}:=B_\epsilon\cap (U^+\setminus V_{2j,\epsilon}),\quad B_{-,\epsilon}:=B_\epsilon\cap (U^-\setminus V_{2j-1,\epsilon}).$$
In order to describe more precisely the connfiguration of these four parts in $W^0$, let us first recall that the periodic orbit $\widebar\apha_j^m$:
\begin{itemize}
\item[--] intersects the torus $T_{2j-1}^m$ at a single point $\bar q_{2j-1}^m\in \pi_\psi^m(D_{2j-1}^s)\cap \pi_\psi^m(D_{2j-1}^u)$,
\item[--] intersects the torus $T_{2j}^m$ at a single point $\bar q_{2j}^m\in \pi_\psi^m(D_{2j}^s)\cap \pi_\psi^m(D_{2j}^u)$,
\item[--] does not intersect the torus $T_i^m$ for $i\neq 2j-1,2j$. 
\end{itemize}
We denote $$\bar \bar q_{2j-1}^m:=\bar h_\epsilon(\bar q_{2j-1}^m) \quad\mbox{ and }\quad \bar \bar q_{2j}^m:=\bar h_\epsilon(\bar q_{2j}^m).$$
These two points do not depend on $\epsilon$ since the restriction $\bar h_\epsilon$ to $\pi_\psi^m(\partial U)$ does not depend on this parameter (see Step 1). More precisely, recall that $\bar h_\epsilon$ is induced by a diffeomorphism $h_\epsilon:U\to U$ such that
$$h_\epsilon=\mathrm{Id}\mbox{ on }T_{2j-1}^{out}\mbox{ and }h_\epsilon=\tau_{-1}^{-1}\mbox{ on }T_{2j-1}^{in}.$$ 
Since $D_{2j-1}^u\subset T_{2j-1}^{out}$ and $D_{2j-1}^s\subset T_{2j-1}^{in}$, it follows that 
\begin{eqnarray*}
&&\bar h_\epsilon(\pi_\psi^m(D_{2j-1}^u)) = \pi_\psi^0(h_1(D_{2j-1}^u))=\pi_\psi^0(D_{2j-1}^u)\\
&&\bar h_\epsilon(\pi_\psi^m(D_{2j-1}^s))=\pi_\psi^0(h_1(D_{2j-1}^s))=\pi_\psi^0(\tau_{-1}^{-1}(D_{2j-1}^s))=\tau_{-1}^{-1}(\pi_\psi^0(D_{2j-1}^s))
\end{eqnarray*}
 hence 
 $$\bar \bar q_{2j-1}^m\in \tau_{-1}^{-1}(\pi_\psi^0(D_{2j-1}^s))\cap \pi_\psi^0(D_{2j-1}^u).$$
 And by a similar computation 
 $$\bar \bar q_{2j-1}^m\in \tau_{-1}^{-1}(\pi_\psi^0(D_{2j}^s))\cap \pi_\psi^0(D_{2j}^u).$$
 We denote by  $\ell^s(\bar \bar q_{2j-1}^m)$ the  leaf of the foliation $f^{s,0}_{2j-1}$ containing $\bar \bar q_{2j-1}^m$, and  by  $\ell^s(\bar \bar q_{2j}^m)$ the  leaf of the foliation $f^{s,0}_{2j}$ containing $\bar \bar q_{2j}^m$. Let
 $$I^s(\bar \bar q_{2j-1}^m)=B_\epsilon\cap T_{\psi,2j-1}^0\mbox{ and }I^s(\bar \bar q_{2j}^m)=B_\epsilon\cap T_{\psi,2j}^0.$$ 
We claim that $I^s(\bar \bar q_{2j-1}^m)$ is contained in the leaf $\ell^s(\bar \bar q_{2j-1}^m)$. Indeed, since $h_\epsilon:U\to U$ is the identity on $U\setminus\cup_i V_{i,\epsilon}$, the image of  the foliation $\bar h_\epsilon(\cF_{\psi}^{s,m})$ coincides with the foliation $\cF_\psi^{s,0}$ outside the $\pi_\psi^0(\cup_i V_{i,\epsilon})$. In particular, $B_\epsilon=\bar h_\epsilon(W^s_{loc}(\widebar\apha_{j}^m))$ is contained in a leaf of the foliation $\cF_\psi^{s,0}$ outside $\pi_\psi^0(\cup_i V_i)$. It follows that $I^s(\bar \bar q_{2j-1}^m)$ is contained in a leaf of the foliation $f^{s,0}_{2j-1}$. This means that $I^s(\bar \bar q_{2j-1}^m)$ is a neighborhood of the point $\bar \bar q_{2j-1}^m$ in the leaf  $\ell^s(\bar \bar q_{2j-1}^m)$, as claimed. Then, by adjusting the width of the ribbon $B$ if necessary, we may assume that $I^s(\bar \bar q_{2j-1}^m)$ is a crossbar of the unstable strip $\pi_\psi^0(D_{2j-1}^u)$. By similar arguments,  
$I^s(\bar \bar q_{2j}^m)$ is a neighborhood of the point $\bar \bar q_{2j}^m$ in the leaf  $\ell^s(\bar \bar q_{2j}^m)$ and we may assume that $I^s(\bar \bar q_{2j}^m)$ is a crossbar of the unstable strip $\pi_\psi^0(D_{2j}^u)$. Now we can describe the different parts $B_\epsilon$:
\begin{itemize}
\item[--] Due to the explicit form of the diffeomorphism $h_\epsilon$ (see Step 1), $B_{2j,\epsilon}$ is a straight ribbon joining $I^s(\bar \bar q_{2j}^m)$ to $Y^0_\epsilon\circ \tau_{-1}(I^s(\bar \bar q_{2j}^m)$ in $\pi_\psi^0(V_{2j,\epsilon})$.
\item[--] The ribbon $B_{+,\epsilon}$ is joining $X_1\circ \tau_{-1}(I^s(\bar \bar q_{2j}^m))$ to $I^s(\bar \bar q_{2j-1}^m)$ inside the tunnel $E_j^+$. This ribbon is a neighborhood of the orbit segment joining $X_1\circ \tau_{-1}(\bar \bar q_{2j}^m)$ to  $\bar \bar q_{2j-1}^m$ in a leaf of  $\cF_\psi^{s,0}$.
\item[--] Then $B_{2j-1,\epsilon}$ is a straight ribbon joining $I^s(\bar \bar q_{2j-1}^m)$ to $Y^0_{\psi,\epsilon}\circ \tau_{-1}(I^s(\bar \bar q_{2j-1}^m))$ in $V_{2j-1,\epsilon}$.
\item[--] Finally $B_{-,\epsilon}$ is joining $Y^0_{\psi,\epsilon}\circ \tau_{-1}(I^s(\bar \bar q_{2j-1}^m))$ to $I^s(\bar \bar q_{2j}^m)$ inside the tunnel $E^-_j$. This ribbon is a neighborhood of the orbit segment joining $X_1\circ \tau_{-1}(\bar \bar q_{2j-1}^m)$ to $\bar \bar q_{2j}^m$ in a leaf of  $\cF_\psi^{s,0}$.
\end{itemize}

\begin{figure}[ht]
\centerline{\includegraphics[width=13.5cm]{Decomposition-B.eps}}
\caption{\label{f.decomposition-B}Decomposition of the closed ribbon $B_\epsilon=\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$.}
\end{figure}

\begin{remark}
\label{r.faithful-2}
In Steps 4, 5 and 6, we will describe some isotopies of the closed ribbons $A$ and $B$. These isotopies will be supported in small neighborhoods of the tori $T_{2j-1}^0$ and $T_{2j}^0$.  As a consequence, our figures below represent quite faithfully the isotopies we will consider (see Remark~\ref{r.faithful}). In principle, the isotopies could described by explicit formulas in the $(x,y,t)$ coordinate system used in Step 1, but we thought this would hardly shed any light on the proof. 
\end{remark}

\subsubsection{Step 4. Isotopy from $B_1=\bar h_1(W^s_{loc}(\widebar\apha_j^m)$ to $B=\lim_{\epsilon\to 0} \bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m)$.}
The diffeomorphism $\bar h_\epsilon$ has been defined for every $\epsilon\in (0,1]$. It does not converge towards a diffeomorphism as $\epsilon\to 0$. Nevertheless, using the explicit definition of $\bar h_\epsilon$, one may easily observe that the closed ribbon $B_\epsilon=\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$ converges, as $\epsilon$ goes to $0$, to a closed ribbon $B$ which is isotopic to $B_1$. Moreover, the decomposition $B_\epsilon=B_{\epsilon,2j}\cup B_{\epsilon,+}\cup B_{\epsilon,2j-1}\cup B_{\epsilon,-}$ converges to a decomposition $B=B_{2j}\cup B_+\cup B_{2j-1}\cup B_-$ of the ribbon $B$. More precisely:
\begin{itemize}
\item[--] $B_{2j}$ is a straight ribbon joining the arc $I^s(\bar \bar q_{2j}^m)$ to the arc $\tau_{-1}(I^s(\bar \bar q_{2j}^m))$ in the torus $T_{2j}^0$;
\item[--] $B_+$ is joining the arc $\tau_{-1}(I^s(\bar \bar q_{2j}^m))$ to the arc $I^s_{\bar \bar q_{2j-1}^m}$ inside the tunnel $E_j^+$; 
it is  a neighborhood of the orbit segment joining $\tau_{-1}(\bar q_{2j}^m)$ to $\bar q_{2j-1}^m$ in a leaf of $\cF_\psi^{s,0}$; 
\item[--] $B_{2j-1}$ is a straight ribbon joining the arc $I^s(\bar q_{2j-1}^m)$ to the  arc $\tau_{-1}(I^s(\bar q_{2j-1}^m))$ in $T_{2j-1}^0$;
 \item[--] $B_-$ is joining the arc $\tau_{-1}(I^s(\bar q_{2j-1}^m))$ to the arc $I^s_{\bar q_{2j}^m}$ inside the tunnel $E_j^-$; it is a neighborhood of the orbit segment joining $\tau_{-1}(\bar q_{2j-1}^m)$ to $\bar q_{2j}^m$ in a leaf of $\cF_\psi^{s,0}$.
\end{itemize}
See figure~\ref{f.first-isotopy-B}.


\begin{figure}[ht]
\centerline{\includegraphics[width=12cm]{First-isotopy-B-1.eps}}
\vspace{0.5cm}
\centerline{\includegraphics[width=12cm]{First-isotopy-B-2.eps}}
\caption{\label{f.first-isotopy-B}Isotopy from $B_1=\bar h_1(W^s_{loc}(\widebar\apha_j^m))$ to $B=\lim_{\epsilon\to 0} \bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$.}
\end{figure}

\subsubsection{Step 5. Isotopy from $B=\lim_{\epsilon\to 0}\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$ to a ribbon $B'$.}
In the preceding step, we have described a decomposition $B=B_{2j}\cup B_+\cup B_{2j-1}\cup B_-$ of the ribbon $B=\lim_{\epsilon\to 0}\bar h_\epsilon(W^s_{loc}(\widebar\apha_j^m))$. Now, we deform $B$ by isotopy as follows. 

The common end $\tau_{-1}(I^s(\bar q_{2j}^m))$ of the ribbons $B_{2j}$ and $B_+$ is contained in the leaf $\ell^s(\tau_{-1}(\bar q_{2j}^m))$ of the foliation $f^{s,0}_{2j}=\cF_\psi^{s,0}\cap T_{2j}^0$. The leaf $\ell^s(\tau_{-1}(\bar q_{2j}^m))$ goes from one end of the stable strip $\pi_\psi^0(D^s_{2j})$ to the other. We deform $B_{2j}$ and $B_+$ by ``dragging" their common end along the leaf $\ell^s(\tau_{-1}(\bar q_{2j}^m))$, in order to bring it inside the same connected component of $\pi_\psi^0(D^s_{2j})\cap \pi_\psi^0(D^u_{2j})$ as the arc $I^s(q^0_{2j})$. See the upper part of Figure~\ref{f.isotopy-B}. This can be done by a isotopy supported in the collar neighborhood $V_{2j}^\epsilon$ of the torus $T_{2j}^0$, for an arbitrarily small $\epsilon$, which respects the  level sets  $\{t=\mbox{constant}\}$ of the $(x,y,t)$ coordinates system on $V_{2j}^\epsilon$ (see Step 1). Moreover, we can choose an isotopy during which $B_{2j}$ moves inside the torus $T_{2j}^0$, and $B_+$ moves inside the tunnel $E_j^+$ (recall that this tunnel is the forward orbit of the strip $\pi_\psi^0(D^s_{2j})$ in $\pi_\psi^0(U^+)$) and inside a leaf of the foliation $\cF_\psi^{s,0}$. At the end of the isotopy, we obtain two new ribbons $B_{2j}'$ and $B_+'$ depicted on the lower part of Figure~\ref{f.isotopy-B}. Adjusting the width of these ribbons if necessary, we may assume that their common end is a crossbar of the unstable strip $D^u_{2j}$. 

Notice that the ribbon $B_+'$ is in good position inside the tunnel $E_j^+$. This is a consequence of three facts: first the initial ribbon $B^+$ is in good position since it is a neighborhood of an orbit segment in a leaf of $\cF_\psi^{s,0}$; second the ribbon remains in this leaf of  $\cF_\psi^{s,0}$ and in the tunnel $E_j^+$ all along the isotopy; third the isotopy is supported in the neighborhood $V_{2j}^\epsilon$ and respects the level sets $\{t=\mbox{constant}\}$ of the $(x,y,t)$ coordinates system and $\frac{\partial}{\partial t}$ corresponds to the vector field $(\pi_\psi^0)_*X=Y^0$.  

We deform similarly the ribbons $B_{2j-1}$ and $B_-$ in a small neighborhood of the torus $T_{2j-1}^0$, leading to new ribbons $B_{2j-1}'$ and $B_-'$ (see again Figure~\ref{f.isotopy-B}). By construction, the closed ribbons $B=B_{2j}\cup B_+\cup B_{2j-1}\cup B_-$  and $B'=B_{2j}'\cup B_+'\cup B_{2j-1}'\cup B_-'$ are isotopic.

\begin{figure}[ht]
\centerline{\includegraphics[width=12cm]{Isotopy-B-1.eps}}
\vspace{0.5cm}
\centerline{\includegraphics[width=12cm]{Isotopy-B-2.eps}}
\caption{\label{f.isotopy-B}Isotopy from the closed ribbon $B=B_{2j}\cup B_+\cup B_{2j-1}\cup B_-$ to the closed ribbon $B'=B_{2j}'\cup B_+'\cup B_{2j-1}'\cup B_-'$.}
\end{figure}

\subsubsection{Step 6. Isotopy from the closed ribbon $A=W^s_{loc}(\widebar\apha_j^0)$ to a ribbon $A'$.}
Now we will deform the closed ribbon $A=A_+\cup A_-$ into a closed ribbon $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$ satisfying the following properties:
\begin{itemize}
\item[--] $A_\pm'$ is a ribbon in good position in the tunnel $\pi_\psi^0(E_j^\pm)$, with the same ends as the $B_\pm'$;
\item[--] $A_{2j}'$ is the section of the unstable strip $\pi_\psi^0(D^u_{2j})$ connecting the right end\footnote{We are considering ribbons with one end in the torus $T_{2j-1}^0$ and one end in the torus $T_{2j}^0$. For sake of simplicity, we call the former \emph{the left end} of the ribbon, and the later \emph{the the right end} of the ribbon (because, on our figures, $T_{2j-1}^0$ is on the left and $T_{2j}^0$ on the right).} of $B_-'$ to the right end of  $B_+'$ ;
\item[--] $A_{2j-1}'$ is the section of the unstable strip $\pi_\psi^0(D^u_{2j-1})$ connecting the left end of $B_-'$ to the left end of  $B_+'$.
\end{itemize}
See the left part of Figure~\ref{f.isotopy-A}. Let us describe more precisely the isotopy. Both the right end of $A_-'$ and the right end of $B_-$ are stable crossbars of the unstable strip $\pi_\psi^0(D^u_{2j})$. So we can ``drag" the right end of $A_-$ among cross bars of $D^u_{2j}$ to bring it up to the right end of $B_-'$ (see Figure~\ref{f.isotopy-A}). This can be done by an isotopy supported in the intersection of the tunnel $E_j^-$ and a small collar neighborhood of $T^{2j}_0$ in $\pi_\psi^0(U^-)$ (recall that $E_j^+$ is the backward orbit of the unstable strip $\pi_\psi^0(D_{2j}^u)$ in $\pi_\psi^0(U^-)$). Moreover this can be done by an isotopy among ribbons that are in good position inside $E_j^-$(recall that, at the beginning of the isotopy, $A^-$ is a piece of local stable manifold, hence is in good position). Now, the right end of $A_+$ and the right end of $B_+$ are contained in the same connected component of $\pi_\psi^0(D_{2j}^u)\cap \pi_\psi^0(D_{2j}^s)$, and both of them are stable crossbars of the unstable strip $D_{2j}^u$. So we can drag the right end of $A_+$ inside  $\pi_\psi^0(D_{2j}^u)\cap \pi_\psi^0(D_{2j}^s)$, among crossbars of $\pi_\psi^0(D^u_{2j})$, to bring it up to the right end of $B_+'$. This can be done by an isotopy among ribbons in good position inside the tunnel $\pi_\psi^0(E_j^+)$(recall that $\pi_\psi^0(E_j^+)$ is the forward orbit of the stable strip $\pi_\psi^0(D^s_{2j})$ in $\pi_\psi^0(U^+)$). At this stage, we have explained how to move the right ends of $A_-$ and $A_+$ up to the right ends of $B_-'$ and $B_+'$, by isotopies of $A_-$ and $A_+$. But such isotopies move the right ends of $A_-$ and $A_+$ appart from each other, and therefore create a ribbon connecting these two ends. Obviously, at the end of the isotopy, this ribbon is nothing but the segment of the unstable strip $D^u_{2j}$ connecting the right ends of $B_-'$ and $B_+'$; we call it $A_{2j}'$. We perform a similar operation in a neighborhood the torus $T_{2j-1}^0$ to bring the lefts ends of $A_-$ and $A_+$ towards the ends of $B_-'$ and $B_+'$. At the end of the day, we obtain that the closed ribbon $A=W^s_{loc}(\widebar\apha_j^0)$ is isotopic to a closed ribbon $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$ where $A_\pm'$, $A_{2j-1}'$ and $A_{2j}'$ satisfy the properties announced above (see the lower part of Figure~\ref{f.isotopy-A}).

\begin{figure}[ht]
\centerline{\includegraphics[width=12cm]{Isotopy-A-1.eps}}
\vspace{0.5cm}
\centerline{\includegraphics[width=12cm]{Isotopy-A-2.eps}}
\caption{\label{f.isotopy-A}Isotopy between $A=A_+\cup A_-$ and $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$.}
\end{figure}

\subsubsection{Step 7. Isotopy between $A'$ and $B'$.}
We will now prove that the ribbons $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$ and $B'=B_{2j}'\cup B_+'\cup B_{2j-1}'\cup B_-'$ are isotopic. Recall that $A_+'$ and $B_+'$ are two ribbons with the same ends. Both $A_+'$ and $B_+'$ are contained in the tunnel $\pi_\psi^0(E_j^+)$, and are in good position inside this tunnel. By the observation at the end of our preliminaries, it follows that $A_+'$ and $B_+'$ are isotopic (with fixed ends). By a similar argument, the ribbons $A_-'$ and $B_-'$ are isotopic with fixed ends. 

So we are left to compare the closed ribbons $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$  and $B_{2j}'\cup A_+'\cup B_{2j-1}'\cup A_-'$, this is equivalent to understand what happens when we replace $A_{2j}'$ by $B_{2j}'$ and replace $A_{2j-1}'$ by $B_{2j-1}'$ in the closed ribbon $A'$. Let us first observe that the core of the closed ribbon $A_{2j}'\cup B_{2j}'$ is homotopic to $0$ in the torus $T_{2j}^{in}$. 


%\begin{remark}
%The following observation will be useful later: \emph{Let $a$ be a path joining a point $q'\in \tau_{-1}^{-1}(L_{2j})$ to a point $q\in R_{2j}$ in the  unstable strip $\varphi^0(D_{2j}^{u})$, and $b$ be a path joining  $q$ to $\tau_{-1}(q')\in L_{2j}$ in the stable strip $D_{2j}^{u}$. Then $a\cdot b$ is homotopic to the straight horizontal path joining  $q'$ to $\tau_{-1}(q')$.} Indeed, let us first observe that the homotopy class of the path $a\cdot b$ is well-defined, by simple connectedness of the strips. Now observe that the translation $\tau_{-1}$ is the product of the symmetry with respect to the leaf  $c_{2j}^{0,s}$ and the symmetry with respect to the leaf $\varphi^0(c_{2j}^{1,u})$. It follows that $R_{2j}$ is the image of $\tau_{-1}^{-1}(L_{2j})$ under the symmetry with respect to $c_{2j}^{0,s}$. This symmetry leaves the strip $\varphi^0(D_{2j}^u)$ invariant. If follows that we can choose the path $a$ to be symmetric with respect to $c_{2j}^{0,s}$. Similarly, we can choose $b$  to be symmetric with respect to $\varphi^0(c_{2j}^{1,u})$. The total variation of the vertical coordinate $y$ along such symmetric path is equal to zero. Hence, $a\cdot b$ is homotopic to a straight horizontal path.
%\end{remark}



Recall that our figures depict faithfully the situation close to $T_{2j-1}^0$ and $T_{2j}^0$, since we have a coordinates system where the flow and the foliations are very simple and fully explicit (see Remarks~\ref{r.faithful} and~\ref{r.faithful-2}). Observing carefully Figure~\ref{f.half-twists}, we see replacing $A_{2j-1}'$ by $B_{2j-1}'$ amounts to a left-handed half-twist, whereas replacing $A_{2j}'$ by $B_{2j}'$ amounts to a right-handed half-twist. These two half-twists cancel each other out, hence $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$  is isotopic to $B_{2j}'\cup A_+'\cup B_{2j-1}'\cup A_-'$. 

We conclude that the ribbons $A'=A_{2j}'\cup A_+'\cup A_{2j-1}'\cup A_-'$ and $B'=B_{2j}'\cup B_+'\cup B_{2j-1}'\cup B_-'$ are isotopic. 

\begin{figure}[ht]
\centerline{\includegraphics[width=12cm]{Half-twists.eps}}
\caption{\label{f.half-twists}Replacing $A_{2j-1}'$ by $B_{2j-1}'$ (resp. $A_{2j}'$ by $B_{2j}'$) is equivalent to a left-handed (resp. right-handed) half-twist. }
\end{figure}

\subsubsection{End of the proof of Proposition~\ref{p.h1}.}
Putting together steps 4 to 7, we conclude that the closed ribbons  $A=W^s_{loc}(\widebar\apha_j^0)$ and $B_1=\bar h_1(W^s_{loc}(\widebar\apha_j^m))$ are isotopic for $j\leq 2m$. Observe that the isotopy we have described is supported in the union of the tunnel $E_j^+$, the tunnel $E_j^-$, a small tubular neighborhood of the torus $T_{2j-1}^0$ and a small tubular neighborhood of the torus $T_{2j}^0$. In particular, the isotopies corresponding to the different integers $j\in\{1,\dots,2m\}$ have disjoint supports. Also recall that the closed ribbons  $W^s_{loc}(\widebar\apha_j^0)$ and $\bar h_1(W^s_{loc}(\widebar\apha_j^m))$ are equal for $j\geq 2m$. We conclude that the ribbon links $W^s_{loc}(\widebar\apha_0^0)\cup\dots\cup W^s_{loc}(\widebar\apha_{2n}^0)$ and $\bar h_1(W^s_{loc}(\widebar\apha_0^m))\cup\dots\cup\bar h_1(W^s_{loc}(\widebar\apha_{2n}^m))$ are isotopic and Proposition~\ref{p.h1} is proved. This concludes the proof of Theorem~\ref{t.con}.


